Anytime-Lidar: Deadline-aware 3D Object Detection

In this work, we present a novel scheduling framework enabling anytime perception for deep neural network (DNN) based 3D object detection pipelines. We focus on computationally expensive region proposal network (RPN) and per-category multi-head detector components, which are common in 3D object detection pipelines, and make them deadline-aware. We propose a scheduling algorithm, which intelligently selects the subset of the components to make effective time and accuracy trade-off on the fly. We minimize accuracy loss of skipping some of the neural network sub-components by projecting previously detected objects onto the current scene through estimations. We apply our approach to a state-of-art 3D object detection network, PointPillars, and evaluate its performance on Jetson Xavier AGX using nuScenes dataset. Compared to the baselines, our approach significantly improve the network's accuracy under various deadline constraints.

==> sections/figs/edge_prob.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.70\linewidth]{figures/edge_probability_light.pdf}
	\caption{Impact of edge probability on virtual gang formation for lightly parallel tasksets}
	\label{fig:ev-edgeprob}
\end{figure}

==> sections/figs/sched_plot_p0.tex <==
\begin{figure*}[t]
    \centering % <-- added
\medskip
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/light_e0_rr.pdf}
  \caption{Lightly Parallel}
  \label{fig:4}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/mixed_e0_rr.pdf}
  \caption{Mixed}
  \label{fig:5}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/heavy_e0_rr.pdf}
  \caption{Heavily Parallel}
  \label{fig:6}
\end{subfigure}
\caption{Schedulability plots for tasksets containing independent tasks ($P(e) = 0$) on 8 cores.}
%Dashed lines are used when interference is not considered. For RT-Gang, because only one task can be scheduled at a time, interference cannot occur by design (thus no dashed lines)}
% \vspace*{-5mm}
\label{fig:sim-p0}
\end{figure*}

==> sections/figs/sched_plot_p25.tex <==
\begin{figure*}[t]
    \centering % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/light_e25_rr.pdf}
  \caption{Lightly Parallel}
  \label{fig:1}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/mixed_e25_rr.pdf}
  \caption{Mixed}
  \label{fig:2}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/heavy_e25_rr.pdf}
  \caption{Heavily Parallel}
  \label{fig:3}
\end{subfigure}
\caption{Schedulability plots for tasksets with precedence constraints ($P(e) = 0.25$) on 8 cores}
% \vspace*{-5mm}
\label{fig:sim-p25}
\end{figure*}

==> sections/figs/smt_timing.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[height=4.5cm, width=0.75\linewidth]{figures/smt_timing_box.pdf}
	\caption{Comparison of SMT and heuristic virtual gang formation runtime. In each box, the orange line represents the median value. The box represents the interquartile range (Q2-Q3). The lower and upper whiskers mark the 5 percentile and the 95 percentile values respectively.}
	\label{fig:smt-time}
\end{figure}
